Evaluating stochastic seeding strategies in networks

When trying to maximize the adoption of a behavior in a population connected by a social network, it is common to strategize about where in the network to seed the behavior, often with an element of randomness. Selecting seeds uniformly at random is a basic but compelling strategy in that it distributes seeds broadly throughout the network. A more sophisticated stochastic strategy, one-hop targeting, is to select random network neighbors of random individuals; this exploits a version of the friendship paradox, whereby the friend of a random individual is expected to have more friends than a random individual, with the hope that seeding a behavior at more connected individuals leads to more adoption. Many seeding strategies have been proposed, but empirical evaluations have demanded large field experiments designed specifically for this purpose and have yielded relatively imprecise comparisons of strategies. Here we show how stochastic seeding strategies can be evaluated more efficiently in such experiments, how they can be evaluated "off-policy" using existing data arising from experiments designed for other purposes, and how to design more efficient experiments. In particular, we consider contrasts between stochastic seeding strategies and analyze nonparametric estimators adapted from policy evaluation and importance sampling. We use simulations on real networks to show that the proposed estimators and designs can increase precision while yielding valid inference. We then apply our proposed estimators to two field experiments, one that assigned households to an intensive marketing intervention and one that assigned students to an anti-bullying intervention.

==> figures/macros.tex <==

\usepackage{amsmath,amsthm,amssymb,eurosym}
\usepackage{enumerate}
\usepackage{graphicx}
%\usepackage{cite}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{titlesec}
\usepackage[OT2,T1]{fontenc} 
\usepackage[russian,american]{babel} 
\usepackage{float}
\usepackage{bbm}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{color}
\usepackage{soul} %for highlighting
\usepackage{wrapfig}
\usepackage{verbatim}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{framed} % for shaded boxes
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{csquotes} % for block quotes
\usepackage{url}
\usepackage{chngcntr}


%~~~~~~~~~~~~~~~~
% Commonly Used Letters
%~~~~~~~~~~~~~~~~
\newcommand{\R}{\mathbb{R}} 	% real numbers	
\newcommand{\C}{\mathbb{C}} 	% complex numbers	
\newcommand{\Z}{\mathbb{Z}} 	% integers
\newcommand{\Q}{\mathbb{Q}} 	% rational numbers
\newcommand{\N}{\mathbb{N}} 	% natural numbers	



\renewcommand{\P}{\mathbf{P}} 	% probability
\newcommand{\E}{\mathbf{E}} 	% expectation
\newcommand{\V}{\mathbf{V}} 	% variance
\newcommand{\bias}{\operatorname{Bias}}   % bias
\newcommand{\var}{\operatorname{Var}}   % variance
\newcommand{\Var}{\operatorname{Var}}   % variance
\newcommand{\cov}{\operatorname{Cov}} 	% covariance
\newcommand{\Cov}{\operatorname{Cov}}   % covariance
\newcommand{\Corr}{\operatorname{Corr}} % correlation

%~~~~~~~~~~~~~~~~
% Calligraphic Letters
%~~~~~~~~~~~~~~~~
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cV}{\mathcal{V}}
%~~~~~~~~~~~~~~~~
% Blackboard or Bold Letters
%~~~~~~~~~~~~~~~~
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\I}{\mathbb{bI}}  % indicator variable
\newcommand{\one}{\mathbbm{1}}  % indicator variable
\renewcommand{\S}{\mathbb{bS}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bV}{\mathbb{V}}

%~~~~~~~~~~~~~~~
% Distributions
%~~~~~~~~~~~~~~~
\def\Gsn{\mathcal{N}}
\def\ber{\textnormal{Ber}}
\def\bin{\textnormal{Bin}}
\def\unif{\textnormal{Unif}}
\def\mult{\textnormal{Mult}}
\def\NegMult{\textnormal{NegMult}}
\def\Dir{\textnormal{Dir}}
\def\bet{\textnormal{Beta}}
\def\pois{\textnormal{Pois}}
\def\HypGeo{\textnormal{HypGeo}}
\def\GEM{\textnormal{GEM}}
\def\BP{\textnormal{BP}}
\def\DP{\textnormal{DP}}
\def\BeP{\textnormal{BeP}}
\def\Exp{\textnormal{Exp}}
\def\gam{\textnormal{Gamma}}

\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\+}[1]{\mathbf{#1}}
\newcommand{\vectsym}[1]{\boldsymbol{#1}}

\newcommand{\note}[1]{\textcolor{red}{\textbf{[#1]}}}

\newcommand{\ip}[2]{\left \langle #1, #2 \right\rangle}
\newcommand{\norm}[1]{\left \lVert #1 \right \rVert}
\newcommand{\abs}[1]{\left \lvert #1 \right \rvert}

\newcommand{\ds}{\displaystyle}
\newcommand{\ep}{\varepsilon}

\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\on}[1]{\operatorname{#1}}

\newcommand{\tr}{\on{tr}} % trace

%~~~~~~~~~~~~~~~~
% Some abbreviations
%~~~~~~~~~~~~~~~~
\newcommand{\plim}{\stackrel{P}{\to}} % convergence in probability
\newcommand{\pto}{\stackrel{p}{\to}}
\newcommand{\wlim}{\Rightarrow} % weak convergence
\newcommand{\wto}{\Rightarrow}
\newcommand{\asto}{\stackrel{\text{a.s.}}{\to}} %a.s. convergence
\newcommand{\lpto}[1]{\stackrel{L^#1}{\to}} %L^p convergence


\newcommand{\io}{\text{ i.o.}} 	%infinitely often
\newcommand{\fo}{\text{ f.o.}} 	%infinitely often
\newcommand{\sumin}{\sum_{i=1}^n} 	%sum from i=1 to n
\newcommand{\pderiv}[1]{\frac{\partial}{\partial #1}}	%partial derivative
\newcommand{\equaldist}{\stackrel{\mathcal{D}}{=}}  %equal in distribution
\newcommand{\eqlaw}{\stackrel{\mathcal{L}}{=}} %equal in law
%
\newcommand{\defeq}{\stackrel{\text{def}}{=}}  %define something
\newcommand{\seteq}{\stackrel{\text{set}}{=}}  %define something
%
\newcommand{\iid}{\stackrel{\text{iid}}{\sim}} % independent and identically distributed
\newcommand{\ind}{\stackrel{\text{ind}}{\sim}} % just independent
%



%New theorem definitions
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
%
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{remarks}{Remarks}

